Thread and Memory-Safe Programming with CLASS

CLASS is a proof-of-concept general purpose linear programming language, flexibly supporting realistic concurrent programming idioms, and featuring an expressive linear type system ensuring that programs (1) never misuse or leak stateful resources or memory, (2) never deadlock, and (3) always terminate. The design of CLASS and the strong static guarantees of its type system originates in its Linear Logic and proposition-as-types foundations. However, instead of focusing on its theoretical foundations, this paper briefly illustrates, in a tutorial form, an identifiable CLASS session-based programming style where strong correctness properties are automatically ensured by type-checking. Our more challenging examples include concurrent thread and memory-safe mutable ADTs, lazy stream programming, and manipulation of linear digital assets as used in smart contracts.

==> eptcsdata.tex <==
\providecommand{\firstpage}{22}
\providecommand{\publicationstatus}{Farzaneh Derakhshan \& Jan Hoffmann (Eds.): 16th International\\ Workshop on
Programming Language Approaches to Concurrency\\
and Communication-cEntric Software 2025 (PLACES 2025)\\
EPTCS 420, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.420.3}{10.4204/EPTCS.420.3}}
\pdfoutput=1

